Vapnik-Chervonenkis Dimension of Axis-Parallel Cuts

The Vapnik-Chervonenkis (VC) dimension of the set of half-spaces of R^d with frontiers parallel to the axes is computed exactly. It is shown that it is much smaller than the intuitive value of d. A good approximation based on the Stirling's formula proves that it is more likely of the order log\_2(d). This result may be used to evaluate the performance of classifiers or regressors based on dyadic partitioning of R^d for instance. Algorithms using axis-parallel cuts to partition R^d are often used to reduce the computational time of such estimators when d is large.

==> defpoly.tex <==
\newcommand{\Nor}[1]{{\mathcal{N}}(0,{#1})}
\newcommand{\T}[1]{{\mathbb{T}}}
\newcommand{\<}{\preceq}
\newcommand{\ct}[1]{{\mathrm{crit}}_{\alpha}({#1})}
\newcommand{\est}[1]{\hat{s}_{#1}}
\newcommand{\eft}[1]{\hat{f}_{#1}}
%\renewcommand{\limits}{{\limits}}

\def\leq{\leqslant}
\def\Ll{{\mathcal{L}}}
\def\s{\sigma}
\def\pn{\par\noindent}
\def\ni{\noindent}
\def\X{{\mathcal{X}}}
\def\l{\lambda}
\def\a{\alpha}
\def\b{\beta}
\def\d{\delta}
\def\k{\kappa}
\def\vf{\varphi}
\def\f{\psi}
\def\ft{\phi}
\def\v{\varepsilon}
\def\O{\Omega}
\def\g{\gamma}
\def\1{1\!{\rm l}}
\def\esm{\hat{s}_m}
\def\efm{\hat{f}_m}
\def\st{\bar{s}_T}
\def\psm{\bar{s}_m}
\def\Esm{\hat{s}_{{\mathfrak{m}}}}
\def\esI{\hat{s}_I}
\def\Psm{\bar{s}_{{\mathfrak{m}}}}
\def\psI{\bar{s}_I}
\def\bg{\bar{\gamma}}
\def\es{\tilde{s}}
\def\ef{\tilde{f}}
\def\Tf{\widetilde{T}}
\def\T{{\mathcal{T}}}
\def\Sm{{{\mathcal{S}}}_m}
\def\Fm{{{\mathcal{F}}}_m}
\def\Mn{{{\mathcal{M}}}_n}
\def\Em{\mathcal{E}_{\mathfrak{m}}}
\def\EI{\mathcal{E}_I}
\def\Pm{\mathcal{P}_{\mathfrak{m}}}
\def\PI{\mathcal{P}_I}
\def\M{{\mathfrak{M}}_n}
\def\m{\mathfrak{m}}
\def\r{\underline{r}}
\def\crit{{{\mathrm{crit}}}}
\def\critn{{{\mathrm{crit}}}_n}
\def\crita{{{\mathrm{crit}}}_{\alpha}}
\def\V{{\mathrm{Var}}}
\def\C{\mathrm{Cov}}
\def\pen{{{\mathrm{pen}}}_n}
\def\argmin{{\mathop{{\mathrm{argmin}}}}}
\def\argmax{{\mathop{{\mathrm{argmax}}}}}
\def\essinf{\mathop{\mathrm{essinf}}}
\def\esssup{\mathop{\mathrm{esssup}}}
\def\P{{{\mathrm{P}}}}
\def\E{{{\mathbb{E}}}}
\def\R{{\mathbb{R}}}
\def\L{{\mathbb{L}}}
\def\F{{\mathcal{F}}}
\def\S{{\mathcal{S}}}
\def\C{{\mathcal{C}}}
\def\Tn{{\mathcal{T}}_n}
\def\Y{{\mathcal{Y}}}

\newcommand{\h}[1]{\hat{#1}} 
\newcommand{\mb}[1]{{\mathbb{#1}}}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\mf}[1]{\mathfrak{#1}}


\newcounter{rem}
\newcommand{\Rem}{
  \smallskip
  \stepcounter{rem} 
  \pn {\bf Remark \arabic{rem}. }}

\newcommand{\Rems}{
  \smallskip
  \pn {\bf Remark. }}

\newcommand{\bull}[1]{
  \medskip
  \pn {\bf $\bullet$ #1 }
  \pn}

\newcommand{\parbf}[1]{
  \smallskip
  \par {\bf #1 . }}














%%% Local Variables: 
%%% mode: plain-tex
%%% TeX-master: "elag"
%%% End: 

